A Unified Framework of Multi-Stage Multi-Winner Voting: An Axiomatic Exploration

Multi-winner voting plays a crucial role in selecting representative committees based on voter preferences. Previous research has predominantly focused on single-stage voting rules, which are susceptible to manipulation during preference collection. In order to mitigate manipulation and increase the cost associated with it, we propose the introduction of multiple stages in the voting procedure, leading to the development of a unified framework of multi-stage multi-winner voting rules. To shed light on this framework of voting methods, we conduct an axiomatic study, establishing provable conditions for achieving desired axioms within our model. Our theoretical findings can serve as a guide for the selection of appropriate multi-stage multi-winner voting rules.

==> approval.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Theoretical results for approval-based rules}
\label{sec:approval}

In this section, we 
%do a similar thing as in Section~\ref{sec: score} and 
provide an axiomatic study for approval-based rules.
%
We focus on the case when single-round rules satisfy a certain desirable property and investigate whether the property can be preserved in multi-rounds that apply one of the single-round rules in each round.
%
\subsection{Preserving axioms in multi-rounds}
\label{sec:approval_preserve}
%
We find the axioms of Pareto efficiency, committee monotonicity, and justified representation preserved in multi-round approval-based voting, which is formalized as the following theorem.
%
\begin{theorem}[\textbf{Pareto efficiency, committee monotonicity, and justified representation preserve in a multi-round approval-based rule}]
    \label{thm:preserving_approval}
    Let $t \geq 1$ be an integer and $\mathcal{R} = (R_1,R_2,...,R_t)$ be a $t$-round multi-winner approval-based voting rule. If $R_r$ is a single-round $\omega$-Thiele rule that satisfies Pareto efficiency, committee monotonicity, or justified representation for each $r\in[t]$, then $\mathcal{R}$ also satisfies Pareto efficiency, committee monotonicity, or justified representation respectively.
    \end{theorem}
\noindent While Pareto efficiency is often regarded as a minimum requirement when we aim to find the “best" candidates, there are a number of single-round rules that do not meet the requirement.
%
\emph{Approval Chamberlin-Courant}, the $\omega$-Thiele with $\omega(x) = \min(1,x)$, is an example of non-Pareto efficient rules (See~\cite[Proposition A.1]{lackner2020multi}). 
%
Moreover, there are many single-round rules that fail to satisfy the criterion of justified representation, though it is considered to be one of the less stringent definitions of “proportional representation" among several possible options.
%
An example is approval voting, mentioned in Section~\ref{sec:rules and axioms}, which simply selects the candidates approved by most voters~\cite{aziz2017justified}.
%
Despite this, the good news is that we can simply prove by contradiction that a multi-round rule satisfies Pareto efficiency (justified representation) if it is composed of single-round $\omega$-Thiele methods that satisfy Pareto efficiency (justified representation); see proofs in Appendix~\ref{sec:proof_of_approval}.

Committee monotonicity is a very demanding criterion for Thiele methods.
%
We show that only the $\omega$-Thiele methods with linear $\omega$-functions satisfy committee monotonicity (Lemma~\ref{lem:CM_approval}, Appendix~\ref{sec:proof_of_approval}).
%
If a multi-round rule $\mathcal{R}$ is composed of rules that maximize $\sum_{v\in V} |A_v\cap S|$ over possible committees $S$ in each round, it must finally select the candidates approved by most voters after multiple rounds.
%
In fact, the multi-round rule $\mathcal{R}$ produces a ranking of candidates and thus satisfies committee monotonicity by definition.

%if some single-round $\omega$-Thiele methods are Pareto efficient, then the multi-round rule composed of them also satisfies Pareto efficiency.
    %\begin{theorem}[\textbf{Pareto efficiency preserves in a multi-round approval-based rule}]
    %\label{thm:PE}
    %Let $t \geq 1$ be an integer and $\mathcal{R} = (R_1,R_2,...,R_t)$ be a $t$-round multi-winner approval-based voting rule. If $R_r$ is a single-round $\omega$-Thiele rule that satisfies Pareto efficiency for each $r\in[t]$, $\mathcal{R}$ also satisfies Pareto efficiency.
    %\end{theorem}
    %

    % Next, we plan to prove that the axiom of committee monotonicity preserves in multi-round approval-based voting. 
    %
    % We formalize our goal with the following theorem.
    %
    % \begin{theorem}[\textbf{Committee monotonicity preserves in a multi-round approval-based rule}]
    % \label{thm:CM_approval}
    % Let $t \geq 2$ be an integer and $\mathcal{R} = (R_1, R_2, \dots, R_t)$ be a $t$-round approval-based rule. If $R_r$ is a single-round $\omega$-Thiele rule that satisfies committee monotonicity for each $r\in[t]$, $\mathcal{R}$ also satisfies committee monotonicity.
    % \end{theorem}
    %
    

    % Justified representation, requiring that no $\lceil\frac{n}{k}\rceil$ voters are totally unrepresented, is the last preserving axiom for approval-based rules. 
    %
    %\begin{theorem}[\textbf{Justified representation preserves in a multi-round approval-based rule}]
    %\label{thm:JR}
    %
    %Let $t \geq 1$ be an integer and $\mathcal{R} = (R_1,R_2,...,R_t)$ be a $t$-round multi-winner approval-based voting rule. If $R_r$ is a single-round $\omega$-Thiele rule that satisfies justified representation for each $r\in[t]$, $\mathcal{R}$ also satisfies justified representation.
    %\end{theorem}
    %
    % \noindent To prove Theorem~\ref{thm:JR}, we need the following lemma, indicating that a candidate approved by $\lceil\frac{n}{k}\rceil$ voters must be selected by a single-round $\omega$-Thiele that satisfies justified representation.
    %
    % We first need to determine what kind of single-round Thiele methods can satisfy justified representation.
    % \begin{lemma}
    % \label{lem:JR}
    % Let there be a set $V^*\subseteq V$ of $\lceil\frac{n}{k}\rceil$ voters such that $\bigcap_{v\in V^*}A_v \neq \varnothing$. 
    % Let there be a set $V^*\subseteq V$ of $\lceil\frac{n}{k}\rceil$ voters and a candidate $c$ such that $\bigcap_{v\in V^*}A_v = \{c\}$. 
    %
    % If $R$ is a single-round $\omega$-Thiele rule that satisfies justified representation, then all the committees in $R(E, k)$ include at least one of the candidates in $\bigcap_{v\in V^*}A_v$.
    % \end{lemma}
    % \begin{proof}
    % Suppose for the sake of contradiction that a committee $S\in R(E, k)$ does not include any candidate in $\bigcap_{v\in V^*}A_v$.
    % all the committees in $R(E, k)$ do not include $c$.
    
    % Fix a committee $S\in R(E, k)$. 
    % For each candidate $b \in S$, define its marginal contribution as the difference between $score_{\omega}(V, \cdot)$ of $S$ and that of $S\backslash\{b\}$.
    %
    % Observe that if a candidate $c\in\bigcap_{v\in V^*}A_v$ were to be added to the winning set $S$, this would increase $score_{\omega}(V, \cdot)$ by at least $\lceil\frac{n}{k}\rceil\cdot \omega(1)$. Since $c$ is not included in $S$, the marginal contribution of each candidate in $S$ must be greater than or equal to $\lceil\frac{n}{k}\rceil\cdot \omega(1)$.
    
    % Let $m(S)$ denote the sum of marginal contributions of all candidates in $S$. Pick any voter $v\in V$. Let $j = |A_v \cap S|$ and $p_j$ denote the difference between $\omega(j)$ and $\omega(j-1)$. If $j > 0$, this voter contributes exactly $p_j$ to the marginal contribution of each candidate in $A_v \cap S$ and hence her contribution to $m(S)$ is exactly $j\cdot p_j$. We denote by $j_0$ the integer $\arg\max_{j\in [k]}j\cdot p_j$. Then $m(S) \leq n\cdot j_0\cdot p_{j_0}$ and the smallest marginal contribution of any candidate in $S$ is at most $\frac{m(S)}{k} \leq \frac{n}{k}\cdot j_0\cdot p_{j_0}$. Due to that the marginal contribution of any candidate in $S$ is greater than that of $c$, we have
    % $$\frac{n}{k}\cdot j_0\cdot p_{j_0} \geq \frac{m(S)}{k} \geq \left\lceil\frac{n}{k}\right\rceil\cdot p_1,$$
    % which is directly followed by $j_0\cdot p_{j_0} \geq p_1$.
    
    % It suffices to argue that there exists some $(E', k')$ such that $R$ does not output any winning set that provides justified representation, which would lead to a contradiction. We let the candidate set be $C' = \{c_0, c_1, ... , c_{j_0}\}$, $n' = k' = j_0$, and consider the profile where the first voter approves $c_0$, whereas each of the remaining voters approves all of $c_1, \dots, c_{j_0}$. Justified representation requires $c_0$ to be selected, but $R$ selects $\{c_1, \dots, c_{j_0}\}$.
    % \end{proof}
    %
    % \noindent Intuitively, a candidate approved by $\lceil\frac{n}{k}\rceil$ voters is selected in each round by rules satisfying justified representation, then it must be included in the final winning committees. Thus there is no set of $\lceil\frac{n}{k}\rceil$ voters completely unrepresented.
    %
    % Now we can prove Theorem~\ref{thm:JR} with Lemma~\ref{lem:JR} as follows.
    %
    

\subsection{Violating axioms in multi-rounds}
\label{sec:approval_violate}

    We discuss in this part the axioms of candidate monotonicity %(Theorem~\ref{thm:candidate_monotone_approval}) 
    and consistency (Theorem~\ref{thm:violating_approval}).
    % (Theorem~\ref{thm:consistency_approval}).
    %
    It is known that all of the single-round Thiele methods satisfy candidate monotonicity and consistency (e.g., see~\cite{lackner2020multi}).
    % It is known that all single-round Thiele methods satisfy candidate monotonicity (e.g., see~\cite{lackner2020multi}).
    %
    However, a multi-round approval-based rule may not satisfy them even though it is composed of single-round Thiele methods.
    %
    \begin{theorem}[\textbf{Candidate monotonicity and consistency do not preserve in a multi-round approval-based rule}]
    \label{thm:violating_approval}
    Let $t\geq 2$ be an integer and $\mathcal{R}$ be a $t$-round $\omega$-Thiele.
    %
    If for any integer $i \geq 0$, $\omega(i)$ is a rational number and
    \begin{equation}
    \label{eq:violating_approval}
       0\neq\omega(i_0-1) - \omega(i_0-2) \neq \omega(i_0) - \omega(i_0-1) 
    \end{equation}
    holds for some $i_0$ in the function $\omega$, then the $t$-round rule
    $\mathcal{R}$ does not satisfy either candidate monotonicity or consistency.
    \end{theorem}
    \begin{proof}[Proof sketch]
        Our plan is to construct example elections 
        % and corresponding vectors $\vec{v} = (k_1, k_2, \dots, k_t)$ 
        to show that $\mathcal{R}$ does not satisfy the axioms of candidate monotonicity and consistency, respectively. 
        %
        
        To show the non-validity of candidate monotonicity, consider an election that selects $i_0$ candidates from $(i_0+1)$ ones in the $(t-1)$-th round and picks $(i_0-1)$ candidates from $i_0$ ones in the last round.
        %
        Suppose that there remain $a, b, c$ and $(i_0-2)$ dummy candidates 
        % designated as $d_{1},d_2,\dots,d_{i_0-2}$ 
        before the commencement of the $(t-1)$-th round.
        %
        We assume that the dummy candidates receive unanimous approval from all voters, and thus they must be included in the final winning committee of size $i_0-1$.
        %
        Therefore, $\mathcal{R}$ needs to select two candidates from $a, b$ and $c$ first and then select one from the aforementioned two candidates.
        %
        As a result of Ineq.~\ref{eq:violating_approval}, it is possible to construct approval ballots of voters $V$ such that (\romannumeral1) the combination of the $(i_0-2)$ dummy candidates with any two of $a, b, c$ yields the same $score_{\omega}(V, \cdot)$ when considering the selection of $i_0$ candidates; (\romannumeral2) when selecting $(i_0-1)$ candidates, $b$ outperforms $a$, and $c$ strictly dominates $b$.
        %
        Then there must exist a winning committee $S$ in the last round such that $b\in S$.
        %
        However, allowing a voter to provide additional approval for candidate $b$ can break the tie in the $(t-1)$-th round and make $\{b, c\}$ combined with the dummies become the sole winning committee.
        %
        This results in the elimination of $b$ in the last round due to the strict dominance of $c$ over $b$.
        
        Similarly, increasing support for certain candidates by adding a set of voters in favor of them not only affects the candidates themselves with support but also alters the outcome for other candidates.
        %
        Although the candidates receiving additional support may still be elected at first, it is possible for the new members of the winning committee in this round to knock out them in the subsequent rounds.
        %
        Consistency therefore cannot preserve in multi-round voting.
    \end{proof}
    %\begin{theorem}[\textbf{Candidate monotonicity does not preserve in a multi-round approval-based rule}]
    %\label{thm:candidate_monotone_approval}
    %Let $t\geq 2$ be an integer and $\mathcal{R}=R^t$ be a $t$-round approval-based rule, where $R$ is a single-round $\omega$-Thiele rule that satisfies candidate monotonicity.
    %
    %If for any integer $i \geq 0$, $\omega(i)$ is a rational number  and
    %$$0\neq\omega(i_0-1) - \omega(i_0-2) \neq \omega(i_0) - \omega(i_0-1)$$
    %holds for some $i_0$ in the function $\omega$ that parameterizes $R$, the multi-round rule
    %$\mathcal{R}$ is not candidate monotone.
    %\end{theorem}
    %
    %\noindent The other violating axiom is consistency, requiring a rule to arrive at consistent outcomes with respect to disjoint groups. 
    %
    %Although each single-round Thiele method satisfies consistency~\cite{lackner2018consistent}, we construct example elections on which a multi-round rule composed of single-round Thiele methods behaves inconsistently.
    %
    %The examples give proof of the following theorem.
    %\begin{theorem}[\textbf{Consistency does not preserve in a multi-round approval-based rule}]
    %\label{thm:consistency_approval}
    %Let $t\geq 2$ be an integer and $\mathcal{R}=R^t$ be a $t$-round approval-based rule, where $R$ is a single-round $\omega$-Thiele rule that satisfies consistency. If 
    %$$\omega(i_0-1) - \omega(i_0-2) \neq \omega(i_0) - \omega(i_0-1)$$
    %holds for some $i_0$ in the function $\omega$ that parameterizes $R$, the multi-round rule
    %$\mathcal{R}$ does not satisfy consistency.
    %\end{theorem}
    %
